The Panchromatic Hubble Andromeda Treasury V: Ages and Masses of the Year 1 Stellar Clusters

We present ages and masses for 601 star clusters in M31 from the analysis of the six filter integrated light measurements from near ultraviolet to near infrared wavelengths, made as part of the Panchromatic Hubble Andromeda Treasury (PHAT). We derive the ages and masses using a probabilistic technique, which accounts for the effects of stochastic sampling of the stellar initial mass function. Tests on synthetic data show that this method, in conjunction with the exquisite sensitivity of the PHAT observations and their broad wavelength baseline, provides robust age and mass recovery for clusters ranging from $\sim 10^2 - 2 \times 10^6 M_\odot$. We find that the cluster age distribution is consistent with being uniform over the past $100$ Myr, which suggests a weak effect of cluster disruption within M31. The age distribution of older ($>100$ Myr) clusters fall towards old ages, consistent with a power-law decline of index $-1$, likely from a combination of fading and disruption of the clusters. We find that the mass distribution of the whole sample can be well-described by a single power-law with a spectral index of $-1.9 \pm 0.1$ over the range of $10^3-3 \times 10^5 M_\odot$. However, if we subdivide the sample by galactocentric radius, we find that the age distributions remain unchanged. However, the mass spectral index varies significantly, showing best fit values between $-2.2$ and $-1.8$, with the shallower slope in the highest star formation intensity regions. We explore the robustness of our study to potential systematics and conclude that the cluster mass function may vary with respect to environment.

==> phat-v3-results.newtable.tex <==
%\begin{landscape}
\begin{deluxetable*}{ccccccccccccccccccccc} 
\tablecolumns{18} 
\tablecaption{Age-Mass and extinction results from the analysis with discrete cluster models.\label{tab:catalog} }
\tablehead{ 
\colhead{}                            &  
\colhead{}                            &  
\colhead{}                            &  
\multicolumn{5}{c}{A$_V$}             & 
\colhead{}                    & 
\multicolumn{5}{c}{$\log(A/yr)$}      & 
\colhead{}                    & 
\multicolumn{5}{c}{$\log(M/M_\odot)$} \\
\cline{4-8} \cline{10-14} \cline{16-20} \\
\colhead{PCNUM}               & 
\colhead{RA\tablenotemark{1}} & 
\colhead{DEC\tablenotemark{1}}  & 
%av
\colhead{best\tablenotemark{2}} & 
\colhead{p16\tablenotemark{3}}  & 
\colhead{p84}                 & 
\colhead{p2.5}                & 
\colhead{p97.5}               & 
\colhead{}                    & 
%loga
\colhead{best}                & 
\colhead{p16}                 & 
\colhead{p84}                 & 
\colhead{p2.5}                & 
\colhead{p97.5}               & 
\colhead{}                    & 
%logM
\colhead{best}                & 
\colhead{p16}                 & 
\colhead{p84}                 & 
\colhead{p2.5}                & 
\colhead{p97.5}               &
\colhead{cflag}\tablenotemark{4}
}
\startdata 

1       & 11.63827 & 42.19389 & 0.9 & 0.6 & 1.2 & 0.6 & 1.2    & & 6.75    & 6.53    &  6.96    & 6.32    & 6.96   & & 3.18    & 2.35    & 3.45    & 2.35    & 3.73  & 0\\
2       & 11.63714 & 42.20994 & 0.3 & 0   & 0.6 & 0   & 0.6    & & 6.53    & 6.32    &  6.75    & 6.32    & 7.18   & & 3.18    & 2.90    & 3.45    & 2.90    & 3.73  & 0\\
29      & 11.62827 & 42.22423 & 0   & 0   & 0.3 & 0   & 0.3    & & 8.47    & 8.25    &  8.68    & 8.25    & 8.68   & & 3.45    & 3.18    & 3.73    & 3.18    & 3.73  & 0\\
34      & 11.59456 & 42.19844 & 0.3 & 0   & 1.5 & 0   & 2.4    & & 8.68    & 8.04    &  9.11    & 7.39    & 9.33   & & 2.35    & 1.80    & 2.90    & 1.53    & 3.18  & 0\\
35      & 11.62181 & 42.20984 & 0.9 & 0.6 & 1.2 & 0.6 & 1.2    & & 6.96    & 6.53    &  7.18    & 6.53    & 7.18   & & 2.08    & 1.80    & 2.63    & 1.53    & 2.63  & 0\\
...     & ...      & ...      & ... & ... & ... & \multicolumn{10}{c}{\it Full table available as electronic supplement} & ... & ...     & ...     & ...     & \\    
1725    & 11.58850 & 42.25820 & 1.2 & 0.3 & 2.1 & 0   & 2.4    & & 7.61    & 6.75    &  8.25    & 6.10    & 8.47   & & 2.63    & 2.08    & 3.18    & 1.53    & 3.18  & 0\\
1726    & 11.60528 & 42.26594 & 1.8 & 0.9 & 2.1 & 0   & 3      & & 8.90    & 8.68    &  9.33    & 7.18    & 10.1   & & 4.01    & 3.45    & 4.28    & 3.18    & 4.56  & 1\\
1728    & 11.58719 & 42.25828 & 0   & 0   & 1.5 & 0   & 2.4    & & 8.04    & 6.10    &  8.25    & 6.10    & 8.68   & & 2.08    & 1.53    & 2.90    & 1.53    & 3.18  & 0\\


%\hline
%\begin{scriptsize}
%$^{\rm(1)}$ Phat cluster id\\
%$^{\rm(2)}$ Right Ascension\\
%$^{\rm(3)}$ Declination\\
%$^{\rm(4)}$ Phot. Aperture\\
%$^{\rm(5)}$ Half light Radius\\
%$^{\rm(6)}$ Typical Aperture Correction\\
%$^{\rm(7)}$ Cluster Rate score\\
%$^{\rm(8)}$ Absolute vega magnitude\\
%$^{\rm(9)}$ F275W uncertainty\\
%$^{\rm(10)}$ Absolute vega magnitude\\
%$^{\rm(11)}$ F336W uncertainty\\
%$^{\rm(12)}$ Absolute vega magnitude\\
%$^{\rm(13)}$ F475W uncertainty\\
%$^{\rm(14)}$ Absolute vega magnitude\\
%$^{\rm(15)}$ F814W uncertainty\\
%$^{\rm(16)}$ Absolute vega magnitude\\
%$^{\rm(17)}$ F110W uncertainty\\
%$^{\rm(18)}$ Absolute vega magnitude\\
%$^{\rm(19)}$ F160W uncertainty\\
%$^{\rm(20)}$ Prob. of bad fit\\
\tablenotetext{1}{ Significantly more figures are available in the electronic table}
\tablenotetext{2}{ ``best'' represents the triplet which maximize the posterior}
\tablenotetext{3}{  ``pXX'' represents the XX-th percentile of the marginalized posterior }
\tablenotetext{4}{  flag suspicious fit from visual CMD inspection (boolean value)}
\enddata
\end{deluxetable*}
%\end{landscape}
%end of table

